Data augmentation with Mobius transformations

Data augmentation has led to substantial improvements in the performance and generalization of deep models, and remain a highly adaptable method to evolving model architectures and varying amounts of data---in particular, extremely scarce amounts of available training data. In this paper, we present a novel method of applying Mobius transformations to augment input images during training. Mobius transformations are bijective conformal maps that generalize image translation to operate over complex inversion in pixel space. As a result, Mobius transformations can operate on the sample level and preserve data labels. We show that the inclusion of Mobius transformations during training enables improved generalization over prior sample-level data augmentation techniques such as cutout and standard crop-and-flip transformations, most notably in low data regimes.

==> figs/fig-cifar.tex <==
\newcommand{\subfigwidth}{0.092}

\begin{figure}[h!]
\begin{centering}
 \begin{subfigure}{}
   \textbf{CIFAR-10 images under M\"obius transformations} \\
  \end{subfigure}%
   \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img8.png}
  \end{subfigure}%
  \\  
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img8.png}
  \end{subfigure}%
  \\
  \caption{Examples of CIFAR classes \{dog, airplane, horse, automobile, bird, ship, cat\} undergoing different M\"obius transformations (original images have green borders).}
  \label{fig:cifar}
\end{centering}
\end{figure}

==> figs/fig-points.tex <==
{\centering
    \quad \textbf{Original} \quad \quad \textbf{Uninterpolated} \quad \textbf{Interpolated} \\
    \includegraphics[width=.45\columnwidth]{figs/points-mapping/points3.png} \\
    \includegraphics[width=.45\columnwidth]{figs/points-mapping/points4.png} \\
    \includegraphics[width=.45\columnwidth]{figs/points-mapping/points2.png} \\
    \includegraphics[width=.45\columnwidth]{figs/points-mapping/points5.png} \\
    \includegraphics[width=.45\columnwidth]{figs/points-mapping/points1.png} \\
}

==> figs/fig-pull.tex <==
\newcommand{\subfigwidthpull}{0.3}

\begin{figure}[ht]
\begin{centering}
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img2.png}
  \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img3.png}
%   \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img4.png}
  \end{subfigure}%
      \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-unconstrained/img7.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-unconstrained/img8.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img5.png}
  \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img6.png}
%   \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-unconstrained/img4.png}
  \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-unconstrained/img5.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img7.png}
%   \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidthpull\columnwidth]{figs/highres-constrained/img8.png}
  \end{subfigure}%
  \\
  \caption{Examples of M\"obius transformations on an image (original with green border). The transformations result in variations in perspective, orientation, and scale, while still preserving local angles and anharmonic ratios.}
  \label{fig:pull}
\end{centering}
\end{figure}

==> figs/fig-random.tex <==
\newcommand{\subfigwidthhighres}{0.25}

\begin{figure}%
\centering
   \subfigure[Unconstrained M\"obius sampling]{%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img1.png}
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img3.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img6.png}
    \label{fig:random-rand}}%
  \\
    \subfigure[Constrained M\"obius sampling]{%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img1.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img4.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img6.png}
    \label{fig:random-def}}%
  \\
  \caption{Examples of M\"obius transformations sampled randomly in an unrestricted manner that often to preserve labels in~\ref{fig:random-rand}, contrasted with those using our constrained sampling method~\ref{fig:random-def}.}
  \label{fig:random}
\end{figure}

==> figs/graph-increasing.tex <==
\begin{figure*}%
\centering
\textbf{Varying M\"obius representation in data augmentation} \\
\subfigure[CIFAR-10]{%
    \label{fig:graph10}%
    \includegraphics[width=.95\columnwidth]{figs/graph-cifar10.png}}%
\qquad
\subfigure[CIFAR-100]{%
    \label{fig:graph100}%
    \includegraphics[width=.95\columnwidth]{figs/graph-cifar100.png}}%
\caption{Results from increasing M\"obius representation in data augmentation from 10\% to 50\% in 10\% increments, across 5 runs. \textbf{(a)} On CIFAR-10, M\"obius at only 10\% with cutout demonstrates empirically best results. M\"obius on its own performs best at 40\%, though it still performs under cutout alone. \textbf{(b)} On CIFAR-100, M\"obius reaches best performance at 20\% on its own and at 10\% with cutout. On both datasets, M\"obius boosts the performance of cutout when applied together, particularly in small quantities of 10-30\%.}
\label{fig:graph}
\end{figure*}

==> figs/neurips-cifar-tiny.tex <==
\newcommand{\subfigwidthtiny}{0.12}
\newcommand{\subfigwidthcifar}{0.08}

\begin{figure}[ht]
\begin{centering}
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthtiny\columnwidth]{figs/Tiny/fish_trans.png}
  \end{subfigure}%
   \begin{subfigure}{}
    \includegraphics[width=\subfigwidthtiny\columnwidth]{figs/Tiny/penguin_trans.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidthtiny\columnwidth]{figs/Tiny/car_trans.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidthtiny\columnwidth]{figs/Tiny/tower_trans.png}
  \end{subfigure}%
  \caption{M\"obius transformations across different animate classes \{goldfish, penguin\} and inanimate classes \{car, tower\} in Tiny ImageNet.}
%   \caption{M\"obius transformations across different animate and inanimate classes in Tiny ImageNet (left: \{goldfish, car, penguin, tower\}) and CIFAR (right: \{airplane, horse, car, bird, ship\}).}
  \label{fig:tiny}
\end{centering}
\end{figure}

==> figs/neurips-cifar.tex <==
\newcommand{\subfigwidth}{0.096}

\begin{figure}[h!]
\begin{centering}
 \begin{subfigure}{}
   \textbf{CIFAR-10 images under M\"obius transformations} \\
  \end{subfigure}%
   \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/dog/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/airplane/img8.png}
  \end{subfigure}%
  \\
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/horse/img8.png}
  \end{subfigure}%
  \\  
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img-original1.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img2.png}
  \end{subfigure}%
  \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img1.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img3.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img4.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img5.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img6.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img7.png}
  \end{subfigure}%
    \begin{subfigure}{}
    \includegraphics[width=\subfigwidth\columnwidth]{figs/car/img8.png}
  \end{subfigure}%
%   \\
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img-original1.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img2.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img1.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img3.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img4.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img5.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img6.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img7.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/bird/img8.png}
%   \end{subfigure}%
% %   \\
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img-original1.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img2.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img1.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img3.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img4.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img5.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img6.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img7.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/ship/img8.png}
%   \end{subfigure}%
%   \\
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img-original1.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img2.png}
%   \end{subfigure}%
%   \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img1.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img3.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img4.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img5.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img6.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img7.png}
%   \end{subfigure}%
%     \begin{subfigure}{}
%     \includegraphics[width=\subfigwidth\columnwidth]{figs/cat/img8.png}
%   \end{subfigure}%
  \\
  \caption{Examples of CIFAR classes \{dog, airplane, horse, automobile, bird, ship, cat\} undergoing different M\"obius transformations (original images have green borders).}
  \label{fig:cifar}
\end{centering}
\end{figure}

==> figs/neurips-random.tex <==
\newcommand{\subfigwidthhighres}{0.25}

\begin{figure}%
\caption{Examples of M\"obius transformations sampled randomly in an unrestricted manner that often to preserve labels in~\ref{fig:random-rand}, contrasted with those using our constrained sampling method~\ref{fig:random-def}.}
\centering
   \subfigure[Unconstrained M\"obius sampling]{%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img1.png}
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img3.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-unconstrained/img6.png}
    \label{fig:random-rand}}%
  \\
    \subfigure[Constrained M\"obius sampling]{%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img1.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img4.png}%
    \includegraphics[width=\subfigwidthhighres\columnwidth]{figs/highres-constrained/img6.png}
    \label{fig:random-def}}%
  \\
  \label{fig:random}
\end{figure}

==> tables/neurips-policies.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]
\centering
% \caption{M\"obius Compared to Data Augmentation Policies}
\begin{tabular}{P{5cm}P{2cm}P{3cm}}
\Xhline{2\arrayrulewidth}
\textbf{Augmentation Method}  & \textbf{Accuracy} & \textbf{Policy Search Time} (GPU hours) \\
\hline
Crop-and-flip  & 81.9\% & \textbf{0}    \\
M\"obius   & 82.5\% & \textbf{0}   \\
M\"obius + $\text{Cutout}$    & \textbf{83.1\%} & \textbf{0}   \\
AutoAugment  & 82.9\% & 5,000  \\
Fast AutoAugment  & 82.7\% & 3.5  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\newline\newline
\caption{Comparison of M\"obius with and without cutout to that of data augmentation policies on CIFAR-100. Our results suggest that M\"obius with cutout performs similarly to these methods already, and provided that the techniques are complementary, M\"obius can be incorporated into their policy search space for improvement.}
\label{tab:policies}
\end{table*}

% These policies use a variety of data augmentation techniques, including cutout but not M\"obius, and require additional time to search and select, or constrain the search space, of possible augmentations. Nevertheless,

==> tables/neurips-tiny-animal.tex <==
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{model}                                                       & \textbf{animate-acc} & \textbf{animate-std} & \textbf{inanimate-acc} & \textbf{inanimate-std} & \textbf{increase} \\ \hline
tiny\_resnet50\_regular\_1\_best\_model\_at\_epoch\_99.csv           & 58.11\%              & 49.34\%              & 53.59\%                & 49.87\%                & 4.52\%            \\ \hline
tiny\_resnet50\_mix5\_madmissable\_2\_best\_model\_at\_epoch\_99.csv & 64.73\%              & 47.78\%              & 57.01\%                & 49.51\%                & 7.72\%            \\ \hline
tiny\_resnet50\_mix4\_madmissable\_3\_best\_model\_at\_epoch\_99.csv & 67.76\%              & 46.74\%              & 54.01\%                & 49.84\%                & 13.75\%           \\ \hline
tiny\_resnet50\_mix6\_madmissable\_3\_best\_model\_at\_epoch\_97.csv & 62.74\%              & 48.35\%              & 58.18\%                & 49.33\%                & 4.55\%            \\ \hline
tiny\_resnet50\_mix3\_madmissable\_3\_best\_model\_at\_epoch\_97.csv & 59.42\%              & 49.10\%              & 55.88\%                & 49.65\%                & 3.54\%            \\ \hline
tiny\_resnet50\_cutout16\_2\_best\_model\_at\_epoch\_97.csv          & 56.50\%              & 49.58\%              & 54.27\%                & 49.82\%                & 2.23\%            \\ \hline
tiny\_resnet50\_mix4\_rand\_3\_best\_model\_at\_epoch\_97.csv        & 63.90\%              & 48.03\%              & 55.91\%                & 49.65\%                & 8.00\%            \\ \hline
tiny\_resnet50\_mix5\_rand\_2\_best\_model\_at\_epoch\_98.csv        & 64.56\%              & 47.83\%              & 55.67\%                & 49.68\%                & 8.90\%            \\ \hline
tiny\_resnet50\_mix3\_rand\_2\_best\_model\_at\_epoch\_99.csv        & 65.10\%              & 47.66\%              & 55.28\%                & 49.72\%                & 9.82\%            \\ \hline
tiny\_resnet50\_mix6\_rand\_3\_best\_model\_at\_epoch\_99.csv        & 65.26\%              & 47.61\%              & 56.30\%                & 49.60\%                & 8.96\%            \\ \hline
\end{tabular}
\caption{Table for animate vs. inanimate class accuracy changes}
\label{tab:animal-tiny}
\end{table}

==> tables/table-animal.tex <==
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]
\centering
\begin{tabular}{P{3.7cm}P{1.9cm}P{.8cm}P{.3cm}|P{3.7cm}P{1.9cm}P{.8cm}P{.3cm}}
\Xhline{2\arrayrulewidth}
\hline
{\bf Animate Superclass} & {\bf Crop-\&-flip} & {\bf Mobius} & {\contour{black}{$\uparrow$}} & {\bf Inanimate Superclass} & {\bf Crop-\&-flip} & {\bf Mobius} & {\contour{black}{$\uparrow$}} \\
\hline
Aquatic Mammals                & 73.0\%    & 74.4\%  & \checkmark & Flowers  & 86.0\%    & 85.6\%  &   \\\hline
Fish                           & 81.8\%   & 82.4\%  & \checkmark & Food Containers    & 79.6\%   & 80.6\%  & \checkmark  \\\hline
Insects                        & 85.0\%    & 85.8\%  & \checkmark & Fruit and Vegetables   & 86.2\%  & 89.6\%  & \checkmark \\\hline
Large Omnivores and Herbivores & 84.4\%   & 84.8\%  & \checkmark & Household Electrical Device & 86.4\%  & 87.0\% & \checkmark \\\hline
Large Carnivores               & 83.8\%   & 84.4\%  & \checkmark &  Household Furniture   & 86.\%.   & 84.8\%   &    \\\hline
Non-insect Invertebrates       & 81.4\%   & 82.0\%   & \checkmark & Large Man-made Outdoor Things  & 89.8\%   & 89.6\%  &        \\\hline
Medium-sized mammals           & 82.6\%   & 85.2\% & \checkmark & Large Natural Outdoor Scenes & 85.2\%  & 87.2\%  & \checkmark \\\hline
People                         & 64.6\%   & 66.8\%  & \checkmark &  Trees    & 75.8\%   & 74.4\%  &  \\\hline
Small Mammals                  & 74.8\%   & 79.0\%    & \checkmark & Vehicles 1    & 88.6\%   & 90.8\%  & \checkmark \\\hline
Reptiles                       & 73.8\%   & 77.2\%  &   \checkmark      & Vehicles   & 91.8\%   & 90.2\%  &   \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{M\"obius data augmentation consistently improves the accuracy of image classification on animate superclasses (\checkmark on {\contour{black}{$\uparrow$}}), as opposed to inanimate superclasses. This empirical observation suggests that M\"obius transformations, having been studied in animals, are particularly attuned to improving generalization in these classes. Note that this finding is interesting, though by no means definitive or theoretically potent.}
\label{tab:animal}
\end{table*}

==> tables/table-main.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[t]
\centering
\begin{tabular}{P{3.5cm}P{2.5cm}P{3cm}P{2.5cm}P{2.5cm}}
\Xhline{2\arrayrulewidth}
\textbf{Augmentation Method}             & \textbf{Dataset}  & \textbf{Average \# Images Per Class} & \textbf{Total \# Training Images} & \textbf{Accuracy} \\
\hline
Crop-and-flip                         & CIFAR-10  & 5000   & 50k   & 96.47\%   $\pm 0.04$    \\
$\text{Cutout}_{l=16}$          & CIFAR-10  & 5000   & 50k   & 97.13\%   $\pm 0.03$      \\
M\"obius                          & CIFAR-10  & 5000   & 50k   & 96.72\%   $\pm 0.06$    \\
M\"obius + $\text{Cutout}_{l=16}$ & CIFAR-10  & 5000   & 50k   & \textbf{97.19\%}   $\pm \textbf{0.07}$  \\
\hline
Crop-and-flip                         & CIFAR-100 & 600    & 50k   & 81.91\%   $\pm 0.20$      \\
$\text{Cutout}_{l=8}$           & CIFAR-100 & 600    & 50k   & 82.35\%   $\pm 0.19$     \\
M\"obius                          & CIFAR-100 & 600    & 50k   & 82.85\% $\pm 0.31$      \\
M\"obius + $\text{Cutout}_{l=8}$  & CIFAR-100 & 600    & 50k   & \textbf{82.92\%}   $\pm \textbf{0.14}$  \\
\hline
Crop-and-flip                         & CIFAR-10  & 400    & 4k    & 83.98\%    $\pm 0.16$     \\
$\text{Cutout}_{l=16}$          & CIFAR-10  & 400    & 4k    & 85.20\%   $\pm 0.22$     \\
M\"obius                          & CIFAR-10  & 400    & 4k    & \textbf{86.07\%}    $\pm \textbf{0.24}$ \\
M\"obius + $\text{Cutout}_{l=16}$ & CIFAR-10  & 400    & 4k    & 85.70\%  $\pm 0.26$     \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Results of main experiments across 5 runs, on several dataset settings: CIFAR-10, CIFAR-100, and reduced CIFAR-10. M\"obius with cutout outperforms all other conditions, followed closely by M\"obius alone in the CIFAR-100 and reduced CIFAR-10 cases, where the average number of images per class is on the order of hundreds. Next, cutout alone and finally standard crop-and-flip. On CIFAR-10, cutout exceeds M\"obius alone, and both outperform the crop-and-flip baseline. We use the optimal lengths for cutout on each dataset (length 16 for CIFAR-10 and length 8 for CIFAR-100) based on prior work~\cite{devries2017improved}.}
\label{tab:main}
\end{table*}

==> tables/table-policies.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}
\centering
% \begin{tabular}{ccc}
\begin{tabular}{P{2.8cm}P{1.3cm}P{3cm}}
\Xhline{2\arrayrulewidth}
\textbf{Augmentation Method}  & \textbf{Accuracy} & \textbf{Policy Search Time} (GPU hours) \\
\hline
Crop-and-flip  & 81.9\% & \textbf{0}    \\
M\"obius + $\text{Cutout}$    & \textbf{82.9\%} & \textbf{0}   \\
AutoAugment  & \textbf{82.9\%} & 5,000  \\
Fast AutoAugment  & 82.7\% & 3.5  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Comparison of M\"obius with cutout to that of data augmentation policies on CIFAR-100. Our results with M\"obius suggest that M\"obius performs similarly to these methods already, and can be incorporated into their policy search space for improvement.}
\label{tab:policies}
\end{table}
% These policies use a variety of data augmentation techniques, including cutout but not M\"obius, and require additional time to search and select, or constrain the search space, of possible augmentations. Nevertheless,

==> tables/table-random.tex <==
% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}
\centering
\begin{tabular}{ccc}
\Xhline{2\arrayrulewidth}
\textbf{Augmentation Method} & \textbf{Dataset} & \textbf{Accuracy} \\
\hline
Crop-and-flip & C10   & 96.47\%   $\pm 0.04$    \\
M\"obius & C10   & \textbf{96.72\%}   $\pm \textbf{0.06}$    \\
Random M\"obius & C10   & 96.54\%   $\pm 0.06$  \\
\hline
Crop-and-flip & C100  & 81.91\%   $\pm 0.20$      \\
M\"obius & C100  & \textbf{82.85\%} $\pm \textbf{0.31}$      \\
Random M\"obius & C100  & 82.30\%   $\pm 0.11$  \\
\hline
Crop-and-flip & R C10  &  83.98\%    $\pm 0.16$     \\
M\"obius & R C10  &  \textbf{86.07\%}    $\pm \textbf{0.24}$ \\
Random M\"obius & R C10  &  85.54\%  $\pm 0.26$     \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Juxtaposition of model performance using randomly parameterized M\"obius transformations with those using defined ones. M\"obius transformations with random parameters suffers in performance, though still better than the crop-and-flip baseline.}
\label{tab:random}
\end{table}

==> tables/table-tiny-animal.tex <==
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{model}                                                       & \textbf{animate-acc} & \textbf{animate-std} & \textbf{inanimate-acc} & \textbf{inanimate-std} & \textbf{increase} \\ \hline
tiny\_resnet50\_regular\_1\_best\_model\_at\_epoch\_99.csv           & 58.11\%              & 49.34\%              & 53.59\%                & 49.87\%                & 4.52\%            \\ \hline
tiny\_resnet50\_mix5\_madmissable\_2\_best\_model\_at\_epoch\_99.csv & 64.73\%              & 47.78\%              & 57.01\%                & 49.51\%                & 7.72\%            \\ \hline
tiny\_resnet50\_mix4\_madmissable\_3\_best\_model\_at\_epoch\_99.csv & 67.76\%              & 46.74\%              & 54.01\%                & 49.84\%                & 13.75\%           \\ \hline
tiny\_resnet50\_mix6\_madmissable\_3\_best\_model\_at\_epoch\_97.csv & 62.74\%              & 48.35\%              & 58.18\%                & 49.33\%                & 4.55\%            \\ \hline
tiny\_resnet50\_mix3\_madmissable\_3\_best\_model\_at\_epoch\_97.csv & 59.42\%              & 49.10\%              & 55.88\%                & 49.65\%                & 3.54\%            \\ \hline
tiny\_resnet50\_cutout16\_2\_best\_model\_at\_epoch\_97.csv          & 56.50\%              & 49.58\%              & 54.27\%                & 49.82\%                & 2.23\%            \\ \hline
tiny\_resnet50\_mix4\_rand\_3\_best\_model\_at\_epoch\_97.csv        & 63.90\%              & 48.03\%              & 55.91\%                & 49.65\%                & 8.00\%            \\ \hline
tiny\_resnet50\_mix5\_rand\_2\_best\_model\_at\_epoch\_98.csv        & 64.56\%              & 47.83\%              & 55.67\%                & 49.68\%                & 8.90\%            \\ \hline
tiny\_resnet50\_mix3\_rand\_2\_best\_model\_at\_epoch\_99.csv        & 65.10\%              & 47.66\%              & 55.28\%                & 49.72\%                & 9.82\%            \\ \hline
tiny\_resnet50\_mix6\_rand\_3\_best\_model\_at\_epoch\_99.csv        & 65.26\%              & 47.61\%              & 56.30\%                & 49.60\%                & 8.96\%            \\ \hline
\end{tabular}
\caption{Table for animate vs. inanimate class accuracy changes}
\label{tab:animal-tiny}
\end{table}
